A Brief Review of Real-World Color Image Denoising

Filtering real-world color images is challenging due to the complexity of noise that can not be formulated as a certain distribution. However, the rapid development of camera lens pos- es greater demands on image denoising in terms of both efficiency and effectiveness. Currently, the most widely accepted framework employs the combination of transform domain techniques and nonlocal similarity characteristics of natural images. Based on this framework, many competitive methods model the correlation of R, G, B channels with pre-defined or adaptively learned transforms. In this chapter, a brief review of related methods and publicly available datasets is presented, moreover, a new dataset that includes more natural outdoor scenes is introduced. Extensive experiments are performed and discussion on visual effect enhancement is included.

==> Algorithm_MSTSVD.tex <==
\begin{algorithm}[ht]
\caption{MS-TSVD} %Ëã·¨µÄÃû×Ö
{\bf Input:} Color image $\mathcal{A}$, patch size $ps$, local search window size $SR$, number of similar patches $K$, pixels between two adjacent reference patches $N_{step}$.\\
{\bf Output:} Filtered image $\mathcal{A}_c$.\\
{\bf Step 1} (Grouping): For a given reference patch, use nearest neighbour search to stack $K$ similar patches in a fourth-order tensor group $\mathcal{G}$.\\
{\bf Step 2} (Collaborative filtering):\\
 \hspace*{0.2in}(1) Learn factor matrices $\hat{\mathbf{U}}_{row}$ and $\hat{\mathbf{U}}_{col}$ according to (\ref{optimize_hosvd_bdiag_tensor}). Learn group-wise transform $\hat{\mathbf{U}}_{group}$ of $\hat{\mathcal{G}}(:,:,1,:)$ via full PCA, and obtain the core tensor $\hat{\mathcal{C}}$
 via (\ref{mstsvd_core_tensor}).\\
 \hspace*{0.2in}(2) Apply the hard-threshold technique to $\hat{\mathcal{C}}$.\\
 \hspace*{0.2in}(3) Take the inverse transform of (\ref{mstsvd_core_tensor}) to obtain filtered 4D group $\mathcal{G}_{filtered}$.\\
{\bf Step 4} (Aggregation): Averagely write back all image patches in $\mathcal{G}_{filtered}$ to their original locations and obtain Filtered image $\mathcal{A}_c$.
\label{ms-tsvd}
\end{algorithm}

